Rethinking Evaluation of Sparse Autoencoders through the Representation of Polysemous Words

Sparse autoencoders (SAEs) have gained a lot of attention as a promising tool to improve the interpretability of large language models (LLMs) by mapping the complex superposition of polysemantic neurons into monosemantic features and composing a sparse dictionary of words. However, traditional performance metrics like Mean Squared Error and L0 sparsity ignore the evaluation of the semantic representational power of SAEs -- whether they can acquire interpretable monosemantic features while preserving the semantic relationship of words. For instance, it is not obvious whether a learned sparse feature could distinguish different meanings in one word. In this paper, we propose a suite of evaluations for SAEs to analyze the quality of monosemantic features by focusing on polysemous words. Our findings reveal that SAEs developed to improve the MSE-L0 Pareto frontier may confuse interpretability, which does not necessarily enhance the extraction of monosemantic features. The analysis of SAEs with polysemous words can also figure out the internal mechanism of LLMs; deeper layers and the Attention module contribute to distinguishing polysemy in a word. Our semantics focused evaluation offers new insights into the polysemy and the existing SAE objective and contributes to the development of more practical SAEs.

==> figure_and_table/activation_comparison.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \vspace{-5mm}
    \includegraphics[width=0.4\textwidth]{figures/Chance_F1_Precision_Recall_vs_Activation_Function_with_legend.pdf}
    \caption{Cosine distance between LLM activations and SAE features in polysemantic contexts. 
    The histogram compares the distribution of 1 - Cosine Similarity for LLM activations (blue) and SAE features (green), demonstrating that SAE features extract more distinct representations in polysemantic contexts.
    We adopt $R = 128$ and $\text{L}_{1}$ coefficient $\lambda = 0.05$ for the hyperparameters of SAEs.
    }
    \label{fig:SAE vs activation}
    \vspace{-40mm}
\end{wrapfigure}

==> figure_and_table/confusion_matrix.tex <==
\begin{table}[t]
\begin{center}
\caption{Confusion matrix for polysemy detection in SAE evaluation.}
\label{table:confuse matrix}
\scalebox{0.875}{
\begin{tabular}{ccc}
\toprule
 & \textbf{Mono-context} & \textbf{Poly-context} \\
\midrule
\multirow{2}{*}{Same Max Activated Feature} & \redcell{Same meaning, same feature} & \bluecell{Different meaning, same feature} \\
& \redcell{(\textbf{T}rue \textbf{P}ositive)} & \bluecell{(\textbf{F}alse \textbf{P}ositive)} \\
\midrule
\multirow{2}{*}{Different Max Activated Feature} & \bluecell{Same meaning, different feature} & \redcell{Different meaning, different feature} \\
& \bluecell{(\textbf{F}alse \textbf{N}egative)} &  \redcell{(\textbf{T}rue \textbf{N}egative)}  \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}

==> figure_and_table/expand_ratio_acc.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/acc_expand_ratio.pdf}
    \caption{Comparison of Accuracy vs MSE and $\text{L}_0$ for different Expand Ratios ($\text{L}_1$ Coef = 0.05). The left panel shows the relationship between accuracy and mean squared error (MSE), while the right panel presents accuracy versus normalized $\text{L}_0$ sparsity. 
    The markers represent various expand ratios (8, 16, 32, 64, and 128). Higher expand ratios generally show a trend towards better performance, as indicated by the yellow and green markers corresponding to expand ratios of 64 and 128.
    }
    \label{fig:Expand_ratio_acc}
\end{figure}

